Abstract Mathematical morphology based on structuring element: Application to morpho-logic

A general definition of mathematical morphology has been defined within the algebraic framework of complete lattice theory. In this framework, dealing with deterministic and increasing operators, a dilation (respectively an erosion) is an operation which is distributive over supremum (respectively infimum). From this simple definition of dilation and erosion, we cannot say much about the properties of them. However, when they form an adjunction, many important properties can be derived such as monotonicity, idempotence, and extensivity or anti-extensivity of their composition, preservation of infimum and supremum, etc. Mathematical morphology has been first developed in the setting of sets, and then extended to other algebraic structures such as graphs, hypergraphs or simplicial complexes. For all these algebraic structures, erosion and dilation are usually based on structuring elements. The goal is then to match these structuring elements on given objects either to dilate or erode them. One of the advantages of defining erosion and dilation based on structuring elements is that these operations are adjoint. Based on this observation, this paper proposes to define, at the abstract level of category theory, erosion and dilation based on structuring elements. We then define the notion of morpho-category on which erosion and dilation are defined. We then show that topos and more precisely topos of presheaves are good candidates to generate morpho-categories. However, topos do not allow taking into account the notion of inclusion between substructures but rather are defined by monics up to domain isomorphism. Therefore we define the notion of morpholizable category which allows generating morpho-categories where substructures are defined along inclusion morphisms. {A direct application of this framework is to generalize modal morpho-logic to other algebraic structures than simple sets.

==> context.tex <==
\subsection{Over morpholizable categories}

Here, we will define a class of categories, called {\em morpholizable categories}, from which we can generate a complete lattice $\mathcal{C}^\mathcal{I}_c$ whose the morphisms between objects (when lattices are seen as categories) are inclusions. 

\begin{notation}[Functor image]
Given a functor $F : \mathcal{C} \to \mathcal{D}$, let us denote $Im(F)$, called {\bf functor image}, the subcategory of $\mathcal{D}$ whose objects are $F(\mathcal{C})$ and morphisms are $Hom_{Im(F)}$ defined as the least subset of $Hom_\mathcal{D}$ containing $F(Hom_\mathcal{C})$ and closed under composition. 
\end{notation}

\Marc{Sans cette fermeture par composition, on n'assure pas n\'ecessairement que $Im(U_i)$ est une cat\'egorie. Il existe des contre-exemples souvent li\'es \`a des foncteurs surjectifs sur les objets mais pas n\'ecessairement sur les morphismes.}

\begin{definition}[Morpholizable category]
A {\bf morpholizable category} $\mathcal{C}$ is a complete and co-complete category equipped with a family of faithful functors $(U_i)_{i \in I}$ such that:

\begin{itemize}
\item {\em Adjunction.} for every $i \in I$, $\mathcal{C}$ is with two functors $\triangle_i : Im(U_i) \to \mathcal{C}$ and $\nabla_i : Im(U_i) \to \mathcal{C}$ which are, respectively, left-adjunct and right-adjunct to $U_i : \mathcal{C} \to Im(U_i)$. 
\item {\em Preservation of equality.} for all object $c,d \in |\mathcal{C}|$, if for every $i \in I$, $U_i(c) = U_i(d)$, then $c = d$.~\footnote{Given a category $\mathcal{C}$, $|\mathcal{C}|$ refers to the collection of objects of $\mathcal{C}$.}
\end{itemize}
\end{definition}
Of course, $\mathcal{C}$ can be a topos which is often the case (any way this the case for most of the examples developped in this paper). 

\begin{example}
Let us return to the examples that we presented in Section~\ref{topos}.

\begin{itemize}
\item {\bf Sets.} The category $Set$ is obviously morpholizable. This category is well-known to have limits and co-limits. Here, we only have a unique forgetful functor $U : Set \to Set$ defined as the identity. Hence, $\triangle$ and $\nabla$ are also the identity functor, and then they are obviously left and right-adjunct to $U$. Obviously, the preservation of equality property is satisfied.
\item {\bf Graphs.} The category of graphs (directed and undirected) $\mathcal{G}$ is known to have limits and co-limits. We have seen in Example~\ref{example:morpho-categories} that two forgetful functors $U_V$ and $U_E$ can be defined on graphs: in the following of the example, to facilitate the presentation, we use the standard definition of graphs which defines a graph by a paire $(V,E)$ where $V$ is its set of vertices and $E$ its set of edges, rather than the one we followed in the previous section to define them by presheaves. 
\begin{enumerate}
\item the forgetful functor $U_V$ associates to any graph $(V,E)$ its set of vertices $V$. It is obvious to show that $U_V$ is faithful. Here, the category $Im(U_V)$ is the category $Set$. Let us define the functor $\triangle_V$ (resp. $\nabla_V$) which to a set $X$ associates the graph $(X,\emptyset)$ (resp. $(X,E)$ with $E = X \times X$). They are well-known to be left-adjunct and right-adjunct to the forgetful functor $U$. 
\item Here, the forgetful functor $U_E$ associates to any graph $(V,E)$ its set of edges $E$, and to any graph morphism $f : (V,E) \to (V',E')$, the mapping $U(f) : U(E) \to U(E')$ which maps any edge $\{x,y\} \in E$ to $\{f(x),f(y)\} \in E'$. Here, the category $Im(U_E)$ has for objects all the sets of $2$-elements sets, and morphisms are all the mappings $m : S \to S'$ for which there is a unique $f : \bigcup_{s \in S} s \to \bigcup_{s' \in S'} s'$ such that for every $\{x,y\} \in S$, $m(\{x,y\}) = \{f(x),f(y)\}$. It is not difficult to show that $U_E$ is faithful. To define the adjunct functor $\nabla_E$, we have to impose that there does not exist isolated vertex (i.e. for every $x$, there exists at least an edge which contains it). Hence, given a set of edges $E \in Im(U_V)$, $\triangle_E(E) = \nabla_E(E) = (V,E)$ where $V = \bigcup_{e \in E} e$. It is quite direct to show that $\triangle_E$ and $\nabla_E$ are adjunct to $U_E$ because both unit morphisms are the identity. \\ The preservation of equality property is obviously satisfied. 
\end{enumerate}  
\item {\bf Hypergraphs.}  As for graphs, to facilitate the prsenation, we choose to define an hypergraph as a set $V$ whose elements are called {\em vertices} together with a family $E = (E_i)_{i \in I}$ of subsets of $V$ called {\em hyperedges}. A morphism of hypergraphs between $(V,E)$ and $(W,F)$ is then a mapping $f : V \to W$ such that for every $E_i \in E$, $f(E_i) \in F$. If we denote by $\mathcal{H}$ the category of hypergraphs, limits and colimits in $\mathcal{H}$ are defined standardly. As well as for graphs, two forgetful functor $U_V$ and $U_E$ can be defined:

\begin{enumerate}
\item the forgetful functor $U_V$ associates to any hypergraph $(V,E)$ its set of vertices $V$. Here again, it is not difficult to show that $U_V$ is faithful. Let us define the functor $\triangle_V$ (resp. $\nabla_V$) which to a set $X$ associates the hypergraph $(X,\emptyset)$ (resp. $(X,E)$ with $E = \mathcal{P}(X)$). It is not difficult to show that $\triangle_V$ and $\nabla_V$ are respectively, left-adjunct and right-adjunct to $U$.
\item the forgetful functor $U_E$ associates to any graph $(V,E)$ its set of hyperedges $E$, and to any hypergraph morphism $f : (V,E) \to (W,F)$ the mapping $U(f) : E \to F$ which maps for every $i \in I$, $E_i$ to $f(E_i) \in F$. Here, the category $Im(U_E)$ has for objects all the sets of sets, and morphisms are all the mappings $m : S \to S'$ for which there is a unique $f : \bigcup_{s \in S} s \to \bigcup_{s' \in S'} s'$ such that for every $s \in S$, $m(s) = \{f(v) \mid v \in s\}$. It is not difficult to show that $U_E$ is faithful. To define the adjunct functor $\nabla_E$, we have to impose that there does not exist isolated vertex. Hence, given a set of edges $E = (E_i)_{i \in I}$, $\triangle_E(E) = \nabla_E(E) = (V,E)$ where $V = \bigcup_{i \in I} E_i$. It is quit direct to show that $\triangle_E$ and $\nabla_E$ are adjunct to $U_E$ because both unit morphisms are the identity. \\ The preservation of equality property is also here obviously satisfied. 
\end{enumerate} 
\item {\bf Simplicial Complex.} Simplicial complexes are geometrical objects defined by combinatory data. They enable to specify topological spaces of arbitrary
dimensions. Simplicial complexes define particular hypergraphs~\footnote{But unlike the catgory of hypergraphs, the category of simplicial complexes is not a topos but only a quasitopose (i.e. it is locally cartesian closed and the subobject classifier $\Omega$ only classifies strong monomorphisms).}. Indeed, a simplicial complex $K$ consists of a set of vertices $V$ and a set $E$ of subsets of $V$ such that $E$ is closed under subsets, for every $v \in V$, $\{v\} \in E$ and $\emptyset {\not \in} E$. Let us note $\mathcal{K}$ the full subcategory of $\mathcal{H}$ whose the objects are simplicial complexes. It is known that the category of simplicial complexes has limits and colimits for small diagrams. As for hypergraphs, the two forgetful functors  $U_V$ and $U_E$ are defined as for hypergraphs. $\triangle_E$ and $\nabla_E$ are defined as reviously. On the contrary, $\triangle_V$ and $\nabla_V$ requires some slighty modifications. Indeed, given a set $X$, both hypergraphs $(X,\{\{x\} \mid x \in X\})$ and $(X,E)$ with $E = \mathcal{P}(X) \setminus \{\emptyset\}$ are simplicial complexes. Therefore, we define the functor $\triangle_V$ (resp. $\nabla_V$) which to a set $X$ associates the hypergraph $(X,\{\{x\} \mid x \in X\})$ (resp. $(X,E)$ with $E = \mathcal{P}(X)  \setminus \{\emptyset\}$). It is not difficult to show that $\triangle_V$ and $\nabla_V$ are respectively, left-adjunct and right-adjunct to $U_V$.
\end{itemize}
\end{example}

Since $\mathcal{C}$ has limits and co-limits, it has terminal and initial objects which are respectively the limit and the co-limit of the empty
diagram. The initial object is denoted by $\emptyset$, and the terminal one is denoted by $1$. 
 
 \medskip
 By standard results of category theory, the following properties are satisfied:
 
 \begin{proposition}
 \label{standard properties} 
 $\mathcal{C}$ satisfies the three following properties: for every $i \in I$
 \begin{itemize}
 \item $U_i$ reflects monics and epics.
 \item $U_i$ preserves limits and colimits.
 \item the pushout of monics is a monic. By duality, the pullback of monics is a monic. More generally, both limits and colimits of monics are monics.
 \end{itemize}
 \end{proposition} 
 
 \begin{proof}
 \begin{itemize}
 \item A consequence of the fact that $U_i$ is faithful.
 \item A consequence of the fact that $U_i$ has a left-adjoint $\triangle_i$ and a right-adjoint $\nabla_i$.
 \item Let
 
 $$
\xymatrix{
 c \ar[r] \ar[d]_{monic} & d \ar[d]^{f} \\
 c' \ar[r] & d'
  }
$$
be a pushout diagram in $\mathcal{C}$. From the two first properties of Proposition~\ref{standard properties}, each $U_i$ preserves and reflects monics and epics. Therefore, since $U_i$ also preserves pushout (the second property of Proposition~\ref{standard properties}), and since the pushout of monics is monic in $Set$, $U_i(f)$ is monic in $Set$. Since $U_i$ reflects monics, we have that $f$ is monic in $\mathcal{C}$.   The proofs for pullback, limits and colimits are similar. 
 \end{itemize}
 \end{proof} 
 
 \begin{corollary}
 Each $U_i$ preserves and reflects epics and monics.
 \end{corollary}
 
 \begin{proof}
 Follows directly from Proposition~\ref{standard properties}.
 \end{proof}
 
 \begin{definition}[Inclusion]
 \label{inclusion}
 A morphism $m : c \to c'$ is called an {\bf inclusion} when for every $i \in I$ each $U_i(m)$ is a set-theoretical inclusion. We will then denote such an inclusion $c \hookrightarrow d$. And, we will denote $\mathcal{I}$ the class of inclusions of $\mathcal{C}$. 
 \end{definition}
 
 \begin{proposition}
 \label{is a partial order}
 $\mathcal{I}$ is a partial order.
 \end{proposition}
 
 \begin{proof}
 It is sufficient to show that there exists at most an inclusion $c \hookrightarrow d$ between objects, and if there exists an inclusion $d \hookrightarrow c$, then $c = d$.
 
\medskip
Then, let us suppose that there exist two inclusions $m : c \hookrightarrow d$ and $m' : c \hookrightarrow d$ in $\mathcal{C}$. Since each $U_i$ is faithful, we have that $U_i(m) \neq U_i(m')$ as $m \neq m'$ which is not possible.
 
\medskip
Let us suppose that there are both $c \hookrightarrow d$ and $d \hookrightarrow c$. By definition of inclusion, we then have that $U(c) = U(d)$. Since $U$ is faithful, then we have that $c \simeq d$, and then by the preservation of equality condition, we can conclude that $c = d$. 
\end{proof}
 
 As this has already observed in~\cite{DGS91}, the interest of inclusions is that subobjects are morphisms instead of equivalence classes of morphisms. This will allow us to extract for each object $c \in |\mathcal{C}|$ a category which will behave like a complete lattice (see Corollary~\ref{complete lattice}). 
 
\begin{proposition}
\label{is factorizable}
Every morphism $f : c \to d$ in $\mathcal{C}$ can be factorized  uniquely as $i \circ e$ where $i$ is an inclusion and $e$ is an epic.
\end{proposition}
 
\begin{proof}
Let $(d \rightrightarrows d \coprod_c d)$ where $d \coprod_c d$ is the pushout 
 
 $$
\xymatrix{
 c \ar[r]^f \ar[d]_f & d \ar[d] \\
 d \ar[r] & d \coprod_c d
  }
$$
Since $\mathcal{C}$ has limit. Let us denote $Im(f)$ the limit of $(d \rightrightarrows d \coprod_c d)$. By definition of limit, the limit $Im(f)$ comes with a morphism $m : Im(f) \to d$ and by the universality property of limit, we also have a unique  morphism $g : c \to Im(f)$. Since each $U_i$ preserves limit, $(U_i(Im(f)),U_i(m))$ is the limit of $(U_i(d) \rightrightarrows U_i(d) \coprod_{U_i(c)} U_i(d))$ in $Set$, and then $U_i(m) : U_i(Im(f)) \to U_i(d)$ is a monic and more precisely an inclusion, and $U_i(e) : U_i(c) \to U_i(Im(f))$ is a surjection. As each $U_i$ reflects both monics and epics, we can conclude that $m$ is an inclusion and $e$ an epic.
 \end{proof}
 
 Following~\cite{DGS91}, morpholizable category are strongly inclusive. They then satisfy the following properties (see~\cite{DGS91} for their proofs):

 \begin{itemize}
 \item all isomorphisms are identities;
 \item any morphism which is both an inclusion and an epic is an identity;
 \item $\mathcal{I}$ is $\mathcal{I}$-right-cancellable in the sense that if $g \circ f \in \mathcal{I}$ and $g \in \mathcal{I}$, then $f \in \mathcal{I}$;
 \item $\mathcal{E}$ is $\mathcal{E}$-right-cancellable where $\mathcal{E}$ is the class of epics of $\mathcal{C}$ (i.e. $\mathcal{E}^{op}$ is $\mathcal{E}^{op}$-right-cancellable). 
 \end{itemize}
 
 We denote by $\mathcal{C}^\mathcal{I}$ the subcategory of $\mathcal{C}$ where $|\mathcal{C}^\mathcal{I}| = |\mathcal{C}|$ and morphisms are all the inclusions in $\mathcal{I}$. 
 
 \begin{proposition}
 \label{inclusions of limits and colimits}
 In $\mathcal{C}$, limits and colimits of inclusions are inclusions.
 \end{proposition}
 
 \begin{proof}
 In $Set$, it is known that limits and colimits of inclusions are inclusions. As each $U_i$ both preserves limits and colimits, and reflects monics, we can conclude that  limits and colimits of inclusions in $\mathcal{C}$ are inclusions. 
 \end{proof}
 
 Since each $U_i$ reflects monics, $\mathcal{C}^\mathcal{I}$ has also $\emptyset$ as initial object. On the contrary, $\mathcal{C}^\mathcal{I}$ has not necessarily a terminal object. The reason is that for most of morpholizable categories (anyway all the categories presented in this paper), the terminal object $1$ has only one morphism which is the identity $Id_1$. This leads to $U_i(1)$ is a singleton, and then as $U_i$ reflects epics, the unique morphism from any object $c$ to $1$ is also an epic.  Hence, the category $\mathcal{C}^\mathcal{I}$ has limits but not necessarily colimits. On the contrary, for any object $c \in |\mathcal{C}|$, the slice category $\mathcal{C}^\mathcal{I}/c$ has for initial object the inclusion $\emptyset \hookrightarrow c$ and for terminal object the identity $Id_c$. Moreover, as each $U_i$ preserves limits and co-limits, and preserves and reflects monics and then inclusions, limits and co-limits of inclusions are inclusions. We can then conclude that the slice category $\mathcal{C}^\mathcal{I}/c$ has limits and co-limits. It is known that there is a forgetful functor $U_c :  \mathcal{C}^\mathcal{I}/c \to \mathcal{C}$ which maps any inclusion $d \hookrightarrow c$ to $d$ and any inclusion $d \hookrightarrow d'$ in $\mathcal{C}^\mathcal{I}/c$ to itself. This forgetful functor leads to a full subcategory $\mathcal{C}^\mathcal{I}_c$ of $\mathcal{C}^\mathcal{I}$. This subcategory is both complete and co-complete. Hence, given an object $c \in \mathcal{C}$, $\mathcal{C}^\mathcal{I}_c$ is the category whose the objects are all the subobjects and the morphisms are all the inclusions between them. This is on this full subcategory $\mathcal{C}^\mathcal{I}_c$ of $\mathcal{C}^\mathcal{I}$ that we will define and will study the properties of erosion and dilation. 
 
 
 \begin{corollary}
 Limits and colimits (when there exist) in $\mathcal{C}^\mathcal{I}$ are unique.
 \end{corollary}
 
 \begin{proof}
 Results directly from Proposition~\ref{is a partial order}. 
 \end{proof}
 
 \begin{corollary}
 \label{complete lattice}
 The category $\mathcal{C}^\mathcal{I}_c$ is a complete lattice.
 \end{corollary}
 
 \begin{proof}
Each forgetful functor $U_i$ entails that $\mathcal{C}^\mathcal{I}_c$ is a small category. Moreover, the objects in $\mathcal{C}^\mathcal{I}_c$ are ordered by inclusions, and given two objects $d$ and $d'$, the least upper bound (lub) of $d$ and $d'$, denoted $\bigvee \{d,d'\}$, is the coproduct of $d$ and $d'$ in $\mathcal{C}^\mathcal{I}_c$, and the greatest lower bound (glb) of $d$ and $d'$, denoted $\bigwedge \{d,d'\}$, is the unique inclusion pullback of the inclusions $(d \hookrightarrow \bigvee \{d,d'\},d' \hookrightarrow \bigvee \{d,d'\})$. Hence, $\mathcal{C}^\mathcal{I}_c$ is a lattice. Finally, by Proposition~\ref{inclusions of limits and colimits}, this lattice is complete. 
 \end{proof}
 
 \begin{example}
In the category of sets $Set$, given a set $S$, $Set^\mathcal{I}_S$ is the complete lattice $(\mathcal{P}(S),\subseteq)$. \\ In the category of graphs $\mathcal{G}$, given a graph $G = (V,E)$, the category $\mathcal{G}^\mathcal{I}_G$ is the lattice of all subgraphs of $G$ (i.e. all the graphs $G' = (V',E')$ such that $V' \subseteq V$ and $E' \subseteq E$). \\ In the category of hypergraphs $\mathcal{H}$, given a hypergraph $H = (V,(E_i)_{i \in I}$, the category $\mathcal{H}^\mathcal{I}_H$ is the lattice of all sub-hypergraphs of $H$ (i.e. all the hypergraphs $H' = (V',(E'_i)_{i \in I'}$ such that $V' \subseteq V$, $I' \subset I$ and for all $i \in I'$, $E_i = E'_i$). 
\end{example}

\begin{definition}[Complement]
Given $d \in \mathcal{C}^\mathcal{I}_c$, let us denote by $\overline{d}$ the {\bf complement} of $d$ (in $\mathcal{C}^\mathcal{I}_c$) defined by: $\overline{d} = \bigvee \{d' \in |\mathcal{C}^\mathcal{I}_c| \mid \bigwedge \{d,d'\} = \emptyset\}$. 
\end{definition}

\begin{proposition}
The following properties are satisfied:

\begin{itemize}
\item if $d \hookrightarrow d'$, then $\overline{d}' \hookrightarrow \overline{d}$;
\item $\bigvee \{d,\overline{d}\} = c$, and $\bigwedge \{d,\overline{d}) = \emptyset$;
\item $\overline{\overline{d}} = d$.
\end{itemize}
\end{proposition}

\begin{proof}
\begin{itemize}
\item Let us suppose that $d \hookrightarrow d'$. Let us show that for every $d'_1 \in \mathcal{C}^\mathcal{I}_C$ such that $\bigwedge \{d',d'_1\} = \emptyset$, we have that $d'_1 \in \{d_1 \mid \bigwedge \{d,d_1\} = \emptyset\}$. If we suppose that there exists $d'' \neq \emptyset$ such that $d'' = \bigwedge \{d,d'_1\}$, then we have that $d'' \hookrightarrow d'$ and $d'' \hookrightarrow d'_1$ which leads to a contradiction.  \\ Hence, $\overline{d}$ is an upper bound of the set $\{d'_1 \mid \bigwedge \{d',d'_1\} = \emptyset\}$, and then by the universal property of lub we have that $\overline{d}' \hookrightarrow \overline{d}$.
\end{itemize}
\end{proof}

\Marc{Je ne suis pas s\^ur que les deux autres points soient satisfaits ?}

%In the following, all diagrams will be considered in $\mathcal{C}^\mathcal{I}_c$. Threfore, they will defined by a set of objects. Implicitely, they will also contain all the least upper bound and all the greatest lower bound of pairs of objects and  all the inclusions which go with. 




==> structuring-reserve.tex <==
\section{Mathematical morphology based on structuring element over a topos}

In the rest of the article, we suppose a topos $\mathcal{C}$.

\subsection{Erosion and dilation}

\begin{definition}[Structuring element]
A {\bf structuring element} $b : X \to P(X)$ is a morphism of $\mathcal{C}$. 
\end{definition}
From a structuring element $b : X \to P(X)$ the symmetric of $b$ is the morphism $\check{b} : X \to P(X)$ satisfying the two equations:

\begin{enumerate}
\item $\pi_1 \circ \varphi(X,X)(b) = \pi_2 \circ \varphi(X,X)(\check{b})$, and
\item $\pi_2 \circ  \varphi(X,X)(b) = \pi_1 \circ \varphi(X,X)(\check{b})$.
\end{enumerate} 
where $\pi_1 : X \times X \to X$ and $\pi_2 : X \times X \to X$ are the projections on the first and the second argument, respectively.

\medskip
As for mathematical morphology defined over sets, given a structruring element $b : X \to P(X)$, both erosion $\varepsilon[b]$ and dilation $\delta[b]$ are two subobjects of $X$ defined as follows:

\begin{definition}[Erosion]
\label{erosion}
Let $b : X \to P(X)$ be a structuring element. Let $U \stackrel{m}{\hookrightarrow} X$ be a monomorphism. The {\bf erosion of $U$ by the structuring element} $b$, denoted $\varepsilon[b](U)$, is the greatest subobject of $X$ (according the ordering induced by monomorphisms, i.e $\preceq$) such that $\bigvee Im(b \circ \varepsilon[b](U)) \hookrightarrow U$. 
\end{definition}

\begin{definition}[Dilation]
Let $b : X \to P(X)$ be a structuring element. Let $U \hookrightarrow X$ be a monomorphism. The {\bf dilation of $U$ by the structuring element} $b$, denoted $\delta[b](U)$, is the subobject $[(\bigvee Im(b \circ U \hookrightarrow X)) \hookrightarrow X]$. 
\end{definition}

\subsection{Properties}

\begin{theorem}[Distributivity of erosion]
$\varepsilon[b](U \cap V) = \varepsilon[b](U) \cap \varepsilon[b](V)$.
\end{theorem}

\begin{proof}

\end{proof}

\begin{corollary}
If $\mathcal{C}$ is co-complete, then we have: $\varepsilon[b](\bigcap_i U_i) = \bigcap_i \varepsilon[b](U_i)$.
\end{corollary}

\begin{theorem}[Distributivity of dilation]
$\delta[b](U + V) = \delta[b](U) + \delta[b](V)$.
\end{theorem}

\begin{proof}

\end{proof}

\begin{corollary}
If $\mathcal{C}$ is complete, then we have: $\delta[b](\sum_i U_i) = \sum_i \delta[b](U_i)$.
\end{corollary}

\begin{theorem}[Monotony]
If $U \hookrightarrow V$, then we have both:

$$\begin{array}{l}
\varepsilon[b](U) \preceq \varepsilon[b](V) \\ \ \\
\delta[b](U) \preceq \delta[b](V)
\end{array}$$
\end{theorem}

\begin{proof}

\end{proof}

\begin{theorem}[Duality]
Let us suppose that there exists the endofunctor $\_^c : \overline{X}^{op} \to \overline{X}$ which for every object $A \in \overline{X}$ associates the (unique) object $B$ such that $A+B = X$ and $A \cap B = \emptyset$. This endofunctor can be extended to subobjects in $Sub(X)$ as follows: $[U \hookrightarrow X]^c = [U^c \hookrightarrow X]$. Then,, we have:

$$\varepsilon[b](U) = \delta(\check{b})(U^c)^c$$
\end{theorem}

